Long-Baseline Interferometric Multiplicity Survey of the Sco-Cen OB Association

We present the first multiplicity-dedicated long baseline optical interferometric survey of the Scorpius-Centaurus-Lupus-Crux association. We used the Sydney University Stellar Interferometer to undertake a survey for new companions to 58 Sco-Cen B- type stars and have detected 24 companions at separations ranging from 7-130mas, 14 of which are new detections. Furthermore, we use a Bayesian analysis and all available information in the literature to determine the multiplicity distribution of the 58 stars in our sample, showing that the companion frequency is F = 1.35 and the mass ratio distribution is best described as a power law with exponent equal to -0.46, agreeing with previous Sco-Cen high mass work and differing significantly from lower-mass stars in Tau-Aur. Based on our analysis, we estimate that among young B-type stars in moving groups, up to 23% are apparently single stars. This has strong implications for the understanding of high-mass star formation, which requires angular momentum dispersal through some mechanism such as formation of multiple systems.

==> bindata.tex <==
\begin{table}
\centering
\caption{The table of observed companion details. Contrast ratios $(\Delta m)$ are in magnitudes, separations ($\rho$) are in milliarcseconds, Obs refers to observation number, position angles (PA) are in degrees and $^n$ following a star name indicates a new companion. For each target, if more than one useable observation was taken we also provide a final contrast ratio and the separations in the North and East direction with their full covariance matrix (the final column is the correlation between the two separations). The high correlations are due to the fact that the measured separations are, in general, approximately north-south pointing.}
\begin{tabular}{cccccccccccccccccccc}
\hline
Name & Obs & MJD & PA($^\circ$) & $\Delta m$ & $\sigma_{\Delta m}$ & $\rho$ & $\sigma_\rho$ &PA$_f$ &$\sigma_{PA_f}$ &$\Delta m_f $& $\sigma_{\Delta m_f}$ &$\rho_f$&$\sigma_{\rho_f}$& $\rho_N$ & $\sigma_{\rho_N}$ & $\rho_E$ & $\sigma_{\rho_E}$ & COR$_{N,E}$& S$_{\Delta_{m}}$\\ 
\hline
4 Lup$^n$     & 1 & 2455393.012 &    14.5 &  2.27 &  0.05 &     11.24 &      0.10 &  &  &  &  &  &&&&&  &  \\
                & 2 & 2455393.033 &    18.0 &  2.56 &  0.08 &     12.52 &      0.21 &  2.41 &  0.29 &  76 & 2 &    5.56 &  24 & 3 &  0.99 &      23.39 &       3.66 &      -1.00  &\\ 
$\alpha$ Mus$^n$ & 1 & 2455391.86 &   191.9 &  1.47 &  0.17 &     10.09 &      0.09 &  &  &&&&&  &  &  &  &&  \\
         & 2 & 2455391.887 &   185.1 &  2.94 &  0.03 &     12.05 &      0.10 &  132 & 2 & 2.21 &  1.47 & 19.8& 0.9 &    -13.39 &       0.19 &      14.56 &       1.13 &      -0.93 & \\
         & 3 &2455414.868 &   209.5 &  2.70 &  0.03 &     16.26 &      0.10 &  &  &  &  &  & &&&& &&  \\
         & 4 & 2455414.878  &   212.0 &  2.06 &  0.02 &     16.37 &      0.03 &  220&5 &2.38 &  0.63 &   16.5  & 1.2 & -12.69 &       1.30 &     -10.59 &       2.10 &      -1.00 &\\ 
    B Cen$^n$ & 1 &2455391.937 &   186.4 &  0.21 &  0.20 &     13.32 &      0.06 &  &&&&&  &  &  &  &  &  &\\
         & 2 & 2455391.958 &   185.7 &  0.56 &  0.22 &      9.21 &      0.03 &  273.9 & 0.1 & 0.38 &  0.35 &  313 & 5 &   21.71 &       0.52 &    -312.04 &       5.07 &      -1.00 &\\
  $\beta$ Mus$^n$ & 1 & 2455391.863 &   186.9 &  3.20 &  0.02 &     18.32 &      0.02 &  &  &  &&&&&  &  &  &  &\\
         & 2 & 2455391.891 &   193.8 &  3.41 &  0.03 &     15.27 &      0.13 &   133.7& 1.6 &3.31 &  0.21 &   30.6&0.9 &   -21.15 &       0.14 &      22.15 &       1.13 &      -0.99 &\\
  $\delta$ Cen & 1 & 2455392.877 &    18.2 &  2.40 &  0.04 &     13.89 &      0.12 &  &  &  &  &  &  &&&&&&  2.5\\
  $\epsilon$ Cen$^n$ & 1 & 2455392.898 &    11.6 &  3.70 &  0.06 &    109.15 &      0.12 & &&&& &  &  &  &  &  &  &\\
         & 2 & 2455392.904 &    10.5 &  3.47 &  0.06 &    115.99 &      0.12 &  298.9& 0.8 &3.59 &  0.23 &    367 & 8 & 177.47 &       1.67 &    -321.05 &       8.51 &      -1.00 &\\
  $\epsilon$ Lup & 1 & 2455391.974 &   188.7 &  1.60 &  0.05 &     49.30 &      0.08 &  &  &  &  &  &  &  &&&&&\\
         & 2 & 2455391.989 &   219.5 &  1.65 &  0.03 &     49.49 &      0.07 &  204.5&0.2 & 1.62 &  0.05 & 51.2& 0.1&    -46.62 &       0.10 &     -21.28 &       0.17 &      -0.81 &1.48\\
    F Cen$^n$ & 1 & 2455403.924 &   204.3 &  2.19 &  0.12 &      8.81 &      0.09 &  &  &  &  &  &&&&&  &&  \\
         & 2 & 2455403.951 &   208.6 &  1.74 &  0.45 &      9.29 &      0.24 & 242& 8& 1.96 &  0.46 & 11.1& 2.5 &     -5.25 &       1.46 &      -9.78 &       3.15 &      -1.00 & \\
  $\gamma$ Lup & 1 & 2455391.978 &   188.8 &  1.63 &  0.05 &     59.14 &      0.09 &  &  &  &  &  &  &  &&&&&\\
         & 2 &2455403.945&   189.3 &  3.47 &  0.05 &     63.03 &      0.12 &  270.0 & 0.3 & 2.55 &  1.84 &  389 & 15 &      0.10 &       2.34 &    -388.59 &      14.76 &      -1.00 &1.5\\
    J Cen$^n$ & 1 & 2455392.958 &   206.7 &  3.04 &  0.03 &     45.67 &      0.09 &  &  &  &  &  &  &  &&&&&\\
              & 2 & 2455392.981 &   212.3 &  2.83 &  0.06 &     36.37 &      0.15 &  145& 7 &2.78 &  0.41 &  95& 10&   -78.54 &       6.45 &      54.27 &      11.46 &      -1.00 &\\
              & 3 & 2455403.931 &    30.6 &  2.46 &  0.03 &     40.33 &      0.08 &  &  &  &  &  &  &  &&&&&\\
  $\kappa$ Cen & 1 & 2455391.94 &   190.1 &  3.19 &  0.10 &    113.77 &      0.22 &  &  &  &  &  &  &&&&&&  \\
         & 2 & 2455391.962 &   185.8 &  2.67 &  0.11 &    110.04 &      0.21 &  211.9 & 1.5 & 2.93 &  0.51 & 112.5&1.9 &    -103.99 &       0.57 &     -64.74 &       3.94 &      -0.96 &1.8\\
  $\kappa$ Sco & 1 & 2455414.899&   170.4 &  0.80 &  0.02 &      4.68 &      0.03 &  &  &  &  &  &  & &&&&& \\
  $\lambda$ Lup & 1 & 2455404.857&   177.1 &  1.72 &  0.01 &     16.68 &      0.02 &  &  &  &  &  &  &  &&&&&\\
         & 2 &2455404.892 &   183.5 &  1.23 &  0.01 &     28.71 &      0.02 &  258.4 & 0.1  & 1.39 &  0.41 & 110.4&0.4 &      -22.16 &       0.08 &    -108.12 &       0.39 &      -0.66 & 1.0\\
         & 3 &  2455403.977  &   198.4 &  1.21 &  0.01 &     55.11 &      0.02 &  &  &  &  &  &  &  &&&&&\\
   $\mu$ Cen$^n$ & 1 & 2455391.906 &   188.5 &  3.47 &  0.05 &     33.10 &      0.10 &  &  &  &  &  &&&&&&  &  \\
         & 2 & 2455391.918&   183.0 &  3.02 &  0.06 &     23.35 &      0.14 &  260.2& 0.1& 3.25 &  0.44 & 105& 2 &      -17.96 &       0.22 &    -103.77 &       1.79 &      -0.93 &\\
  o Lup & 1 & 2455392.984 &   196.2 &  0.77 &  0.01 &     42.62 &      0.01 &  &  &  &  &  &  & &&&& &0.45\\
$\phi^2$ Lup$^n$ & 1 & 2455393.005 &    15.7 &  2.53 &  0.19 &     25.35 &      0.31 &  &  &  &  &  &&&&&&  &  \\
         & 2 & 2455393.024&    18.8 &  2.18 &  0.05 &     16.78 &      0.07 &  295 & 1& 2.36 &  0.34 &    161.2  &5.5 &   67.58 &       1.88 &    -146.32 &       5.56 &      -1.00 &\\
   $\pi$ Cen & 1 & 2455391.846 &   186.1 &  1.76 &  0.07 &     26.66 &      0.16 &  &  &  &  &  &  &&&&& & \\
         & 2 & 2455391.871 &   191.2 &  0.91 &  0.12 &     34.17 &      0.14 & 258.9& 0.3&  1.34 &  0.85 & 90.2&2.3 &     -17.32 &       0.39 &     -88.55 &       2.38 &      -0.96 & 1.5\\
  $\rho$ Lup$^n$ & 1 & 2455391.93&   187.3 &  1.37 &  0.02 &     15.45 &      0.04 &  &  &  &  &  &  &  &&&&&\\
         & 2 & 2455391.951&   186.2 &  2.04 &  0.03 &     16.12 &      0.06 &  120& 3& 1.70 &  0.67 &  39&3 &    -19.90 &       0.44 &      33.85 &       3.66 &      -1.00 & \\
  $\sigma$ Cen$^n$ & 1 & 2455391.883 &   194.3 &  2.84 &  0.18 &     98.24 &      0.41 &  &  &  &  &  &&&&&&  &  \\
  $\tau^1$ Lup$^n$ & 1 & 2455403.968 &   201.9 &  2.83 &  0.04 &     18.83 &      0.04 &  &  &  &  &  &  &  &&&&&\\
         & 2 & 2455404.85 &   181.2 &  3.07 &  0.04 &     18.07 &      0.05 &  &  &  &  &  &  &  &&&&&\\
         & 3 & 2455404.885 &   187.7 &  2.75 &  0.08 &     18.58 &      0.10 & 197.9& 0.1 &  2.88 &  0.24 &  18.9& 0.1 &    -17.96 &       0.00 &      -5.82 &       0.01 &      -0.76 & \\
  $\tau$ Lib$^n$ & 1 & 2455392.0&   185.6 &  2.60 &  0.04 &     12.35 &      0.10 &  &  &  &  &  &  &  &&&&&\\
  $\tau$ Sco$^n$ & 1 &2455392.027&   232.2 &  3.50 &  0.01 &     20.30 &      0.07 &  &  &  &  &  &  &  &&&&&\\
         & 2 & 2455392.012   &   192.1 &  2.81 &  0.02 &     11.90 &      0.06 &  247.7&0.2 & 3.16 &  0.69 &  21.1&0.1 &    -7.98 &       0.08 &     -19.50 &       0.12 &      -0.72 &\\
   $\delta$ Sco C$^n$ & 1 & 2455392.923&   176.7 &  4.19 &  0.41 &     77.96 &      0.45 &  &  &  &  &  &  &&&&&&  \\
         & 2 & 2455392.941 &   180.0 &  3.60 &  0.28 &     78.83 &      0.29 &  189.3 &6.6 & 3.90 &  0.60 & 79.9&1.6 &      -78.84 &       0.29 &     -12.85 &       9.27 &       0.56 &\\
   $\delta$ Sco B & 1 & 2455392.923 &   176.7 &  1.51 &  0.24 &      8.56 &      0.05 &  &  &  &  &  &  &  &&&&&\\
         & 2 & 2455392.941 &   180.0 &  1.95 &  0.39 &      9.22 &      0.07 &  230.7&3.5 & 1.73 &  0.44 &     14.6 &1.1 &  -9.22 &       0.07 &     -11.27 &       1.37 &       0.82 & 2\\
\hline
\end{tabular}
\label{bintab}
\end{table}


==> observed_stars_old.tex <==
13-Sco & 79404 & 1.53 & 2.92 & 2.98 & 2.96 & 2.73 & 2.21 & 1.62 & 0.84 \\
3-Cen & 67669 & 2.54 & 3.67 & 3.71 & 3.69 & 3.45 & 2.97 & 2.29 & 1.70 \\
4-Cen & 67786 & 1.98 & 3.19 & 3.21 & 3.13 & 2.95 & 2.44 & 1.86 & 1.18 \\
4-Lup & 76945 & 1.92 & 3.16 & 3.21 & 3.17 & 2.98 & 2.44 & 1.84 & 1.12 \\
7-Sco & 78401 & 2.25 & 3.57 & 3.74 & 3.66 & 3.49 & 2.85 & 2.24 & 1.60 \\
G-Cen & 60710 & 2.68 & 3.22 & 2.90 & 3.29 & 3.06 & 2.66 & 2.17 & 1.45 \\
a-Cen & 70300 & 2.20 & 3.14 & 3.11 & 3.11 & 2.91 & 2.48 & 1.86 & 1.30 \\
$\alpha$-Lup & 71860 & 2.86 & 2.42 & 2.94 & 3.19 & 3.01 & 2.68 & 2.24 & 1.45 \\
$\alpha$-Mus & 61585 & 4.23 & 3.69 & 4.64 & 4.22 & 4.74 & 4.25 & 3.83 & 3.14 \\
b-Cen & 71865 & 2.20 & 3.37 & 3.34 & 3.32 & 3.10 & 2.60 & 1.99 & 1.53\\
$\beta$-Cru & 62434 & 2.29 & 1.97 & 2.33 & 2.61 & 2.47 & 2.12 & 1.60 &0.85\\
$\beta$-Lup & 73273 & 3.08 & 4.05 & 4.04 & 4.09 & 3.79 & 3.24 & 2.65 & 2.11 \\
$\beta$-Mus & 62322 & 3.89 & 4.49 & 4.52 & 4.40 & 4.20 & 3.74 & 3.34 & 2.59 \\
$\chi$-Cen & 68862 & 2.11 & 3.10 & 3.20 & 3.08 & 2.91 & 2.41 & 1.79 & 1.21 \\
$\delta$-Cen & 59196 & 3.21 & 3.82 & 3.58 & 3.78 & 3.72 & 3.27 & 2.71 & 1.87 \\
$\delta$-Cru & 59747 & 3.38 & 3.03 & 3.44 & 3.68 & 3.52 & 3.12 & 2.69 & 1.90 \\
$\delta$-Lup & 75141 & 2.44 & 3.37 & 3.35 & 3.27 & 3.15 & 2.70 & 2.01 & 1.53 \\
d-Lup & 76371 & 2.19 & 3.15 & 3.12 & 2.99 & 2.93 & 2.47 & 1.82 & 1.31 \\
e-Lup & 74449 & 1.96 & 3.04 & 3.01 & 2.94 & 2.83 & 2.30 & 1.73 & 1.12 \\
$\epsilon$-Cen & 66657 & 3.67 & 4.16 & 4.06 & 4.32 & 4.04 & 3.55 & 3.06 & 2.30 \\
$\epsilon$-Lup & 75264 & 3.06 & 3.69 & 3.69 & 3.67 & 3.43 & 3.02 & 2.62 & 1.86 \\
$\eta$-Cen & 71352 & 3.12 & 4.14 & 4.22 & 4.28 & 3.86 & 3.35 & 2.76 & 2.10 \\
$\eta$-Lup & 78384 & 3.24 & 3.96 & 4.01 & 4.04 & 3.76 & 3.20 & 2.64 & 1.98 \\
f-Cen & 63945 & 2.80 & 3.34 & 3.16 & 3.37 & 3.18 & 2.76 & 2.22 & 1.65 \\
$\gamma$-Lup & 76297 & 3.96 & 5.08 & 5.05 & 5.06 & 4.75 & 4.30 & 3.51 & 2.63 \\
$\gamma$-Mus & 61199 & 2.48 & 1.81 & 2.98 & 2.18 & 2.92 & 2.61 & 2.29 & 1.66 \\
HR 4549 & 57851 & 2.67 & 1.54 & 3.29 & 2.90 & 3.34 & 2.98 & 2.53 & 1.88 \\
HR 4618 & 59173 & 3.22 & 3.41 & 3.11 & 3.65 & 3.46 & 3.02 & 2.56 & 1.90 \\
HR 4848 & 62327 & 2.92 & 2.59 & 2.98 & 3.23 & 3.09 & 2.70 & 2.28 & 1.56 \\
HR 5543 & 72800 & 1.47 & 2.77 & 2.77 & 2.77 & 2.53 & 2.03 & 1.42 & 0.65 \\
HR 5967 & 78655 & 1.71 & 2.98 & 3.01 & 3.00 & 2.78 & 2.25 & 1.65 & 0.88 \\
$\iota$-Lup & 69996 & 3.13 & 4.06 & 4.04 & 3.98 & 3.88 & 3.29 & 2.68 & 2.06 \\
j-Cen & 57669 & 3.22 & 2.82 & 3.33 & 3.54 & 3.38 & 3.05 & 2.53 & 1.90 \\
$\kappa$-Cen & 73334 & 2.94 & 3.93 & 3.79 & 3.72 & 3.68 & 3.11 & 2.51 & 1.94 \\
$\kappa$-Sco & 86670 & 4.33 & 5.34 & 5.47 & 5.35 & 5.08 & 4.59 & 3.97 & 2.95 \\
$\xi^2$-Cen & 64004 & 3.04 & 3.50 & 3.27 & 3.58 & 3.36 & 2.99 & 2.43 & 1.77 \\
$\lambda$-Cru & 63007 & 2.99 & 2.55 & 3.08 & 3.33 & 3.18 & 2.85 & 2.32 & 1.55 \\
$\lambda$-Lup & 74117 & 3.19 & 4.18 & 4.28 & 4.33 & 4.01 & 3.41 & 2.84 & 2.24 \\
$\mu$01-Cru & 63003 & 2.46 & 1.32 & 2.70 & 2.75 & 2.65 & 2.29 & 1.84 & 1.19 \\
$\mu$02-Sco & 82545 & 2.53 & 3.53 & 3.60 & 3.59 & 3.49 & 3.13 & 2.81 & 2.32 \\
$\mu$-Cen & 67472 & 2.57 & 3.63 & 3.67 & 3.53 & 3.40 & 2.88 & 2.29 & 1.76 \\
$\nu$-Cen & 67464 & 1.37 & 2.85 & 2.91 & 2.85 & 2.65 & 2.14 & 1.54 & 0.00 \\
$o$-Lup & 72683 & 2.71 & 3.71 & 3.69 & 3.63 & 3.47 & 2.93 & 2.29 & 1.73 \\
$\phi^2$-Lup & 75304 & 2.17 & 3.34 & 3.39 & 3.32 & 3.12 & 2.61 & 2.03 & 1.32 \\
$\phi$-Cen & 68245 & 2.12 & 3.04 & 2.90 & 2.79 & 2.90 & 2.34 & 1.82 & 1.15 \\
$\pi$-Cen & 55425 & 2.60 & 3.04 & 2.69 & 3.16 & 3.02 & 2.62 & 2.00 & 1.33 \\
$\pi$-Sco & 78265 & 2.93 & 3.35 & 3.41 & 3.58 & 3.62 & 3.39 & 3.09 & 2.52 \\
$\rho$-Cen & 59449 & 2.15 & 2.68 & 2.30 & 2.77 & 2.63 & 2.18 & 1.62 & 0.90 \\
$\rho$-Lup & 71536 & 2.32 & 3.46 & 3.49 & 3.47 & 3.26 & 2.72 & 2.12 & 1.52 \\
$\rho$-Sco & 78104 & 1.95 & 3.24 & 3.31 & 3.35 & 3.08 & 2.59 & 1.93 & 1.33 \\
$\sigma$-Cen & 60823 & 2.67 & 2.26 & 2.66 & 3.17 & 3.05 & 2.57 & 2.10 & 1.35 \\
$\sigma$-Lup & 71121 & 3.04 & 3.76 & 3.68 & 3.60 & 3.58 & 3.11 & 2.54 & 1.74 \\
$\tau^1$-Lup & 70574 & 3.41 & 4.24 & 4.19 & 4.17 & 3.99 & 3.52 & 2.90 & 2.21 \\
$\tau$-Lib & 76600 & 2.22 & 3.52 & 3.54 & 3.52 & 3.33 & 2.77 & 2.13 & 1.57 \\
$\tau$-Sco & 81266 & 2.91 & 4.01 & 4.00 & 3.97 & 3.75 & 3.49 & 3.35 & 2.68 \\
$\theta$-Lup & 78918 & 1.04 & 2.57 & 2.62 & 2.60 & 2.38 & 1.88 & 1.24 & 0.00 \\
$\upsilon^1$-Cen & 68282 & 2.13 & 3.11 & 3.00 & 2.83 & 2.88 & 2.42 & 1.75 & 1.17 \\
$\zeta$-Cru & 60009 & 2.64 & 2.96 & 2.97 & 3.08 & 2.88 & 2.50 & 1.97 & 1.19 \\
